Joint Unsupervised Learning of Optical Flow and Egomotion with Bi-Level Optimization

We address the problem of joint optical flow and camera motion estimation in rigid scenes by incorporating geometric constraints into an unsupervised deep learning framework. Unlike existing approaches which rely on brightness constancy and local smoothness for optical flow estimation, we exploit the global relationship between optical flow and camera motion using epipolar geometry. In particular, we formulate the prediction of optical flow and camera motion as a bi-level optimization problem, consisting of an upper-level problem to estimate the flow that conforms to the predicted camera motion, and a lower-level problem to estimate the camera motion given the predicted optical flow. We use implicit differentiation to enable back-propagation through the lower-level geometric optimization layer independent of its implementation, allowing end-to-end training of the network. With globally-enforced geometric constraints, we are able to improve the quality of the estimated optical flow in challenging scenarios and obtain better camera motion estimates compared to other unsupervised learning methods.

==> local-definitions.tex <==
% \usepackage{xspace}
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
% \def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
% \def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
% \def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
% \def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
% \def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
% \def\etal{\emph{et al}\onedot}
% Steve prefers non-italicized
\def\eg{{e.g}\onedot} \def\Eg{{E.g}\onedot}
\def\ie{{i.e}\onedot} \def\Ie{{I.e}\onedot}
\def\cf{{c.f}\onedot} \def\Cf{{C.f}\onedot}
\def\etc{{etc}\onedot} \def\vs{{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{{et al}\onedot}
\makeatother

% Maths:
\newcommand{\ddx}[1]{\frac{\text{d} #1}{\text{d}x}}
\newcommand{\dd}[2]{\frac{\text{d} #1}{\text{d} #2}}
\newcommand{\ddinline}[2]{\text{d} #1 / \text{d} #2}
\newcommand{\del}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\deldel}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\deldelm}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}

% Sets:
\newcommand{\sV}{\mathcal{V}}

% \newcommand{\argmin}{\mathop{\textrm{argmin}}}
% \newcommand{\argmax}{\mathop{\textrm{argmax}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator*{\charb}{\rho_c}

% References:
\newcommand{\figref}[1]{Figure~\ref{#1}}


==> table_kitti_w_test.tex <==
% http://pgfplots.sourceforge.net/pgfplotstable.pdf
\begin{table*}[!t]\centering
\caption{Performance comparison on the KITTI 2012 benchmark.
We report the mean End Point Error (EPE) of the predicted optical flow on the training and test sets for all pixels and non-occluded (noc) pixels,
and the Percentage of Improved Instances (PoII) over the baseline model.
EPIFlow and our models were trained on the KITTI VO dataset. 
Parentheses and the suffix -ft indicate that the models were fine-tuned on the data, missing entries (--) indicate that the results were not reported, and bold entries indicate the best results. The arrows ($\downarrow$) / ($\uparrow$) indicate lower / upper is better.
}
\label{tab:kitti}
\newcolumntype{C}{>{\centering\arraybackslash}X}
% \renewcommand*{\arraystretch}{1.3} % Use/adjust if desired
\setlength{\tabcolsep}{0pt} % Use/adjust if desired
\begin{tabularx}{0.25\textwidth}{@{}l l}
    \toprule
    \\
    \addlinespace
    & Method\\
    \midrule
    & EpicFlow \cite{revaud2015epicflow}\\
    \midrule
    \multirow{4}{10pt}{\rotatebox{90}{\small Supervised}}
    &SpyNet-ft \cite{ranjan2017optical}\\
    &FlowNet2-ft \cite{ilg2017flownet}\\
    &PWC-Net \cite{sun2018pwc}\\
    &PWC-Net-ft \cite{sun2018pwc}\\
    \midrule
    \multirow{11}{10pt}{\rotatebox{90}{\small Unsupervised}}
    &UnsupFlownet \cite{jason2016back}\\
    &DSTFlow \cite{ren2017unsupervised}\\
    &DF-Net \cite{zou2018df}\\
    &UnFlow \cite{meister2018unflow}\\
    &OAFlow \cite{wang2018occlusion}\\
    &EPIFlow-F \cite{zhong2019unsupervised}\\
    &EPIFlow-sub-ft \cite{zhong2019unsupervised}\\
    \cmidrule[\lightrulewidth](r{-1.6em}){2-2}
    % \midrule
    &Ours-Baseline\\
    &Ours-ApproxGrad\\
    &Ours-NoPrior\\
    &Ours\\
    % &Ours-FT\\
    \bottomrule
\end{tabularx}%
\pgfplotstabletypeset[
    column type=, % clear defaults
    trim cells=true,
    begin table={\begin{tabularx}{0.75\textwidth}{@{}C C C C C C@{}}},
    end table={\end{tabularx}},
    col sep=comma,
    row sep=newline,
    header=false,
    every head row/.style={
        output empty row,
        before row={
            \toprule
            % \multicolumn{4}{c}{KITTI 2012}\\
            \multicolumn{2}{c}{EPE (all) $\downarrow$} & \multicolumn{2}{c}{EPE (noc) $\downarrow$} & PoII (all) $\uparrow$ & PoII (noc) $\uparrow$\\
            \cmidrule(lr){1-2}
            \cmidrule(lr){3-4}
            \cmidrule(lr){5-5}
            \cmidrule(lr){6-6}
            train & test & train & test & train & train\\
        },
        after row=\midrule,
    },
    every last row/.style={after row=\bottomrule},
    every row no 1/.style={before row=\midrule},
    every row no 5/.style={before row=\midrule},
    every row no 12/.style={before row=\midrule},
    columns/0/.style={column name=,
        string replace={0}{}, % erase ’0’
        fixed zerofill,
        precision=2,
    },
    columns/1/.style={column name=,
        string replace={0}{}, % erase ’0’
        fixed zerofill,
        precision=2,
    },
    columns/2/.style={column name=,
        string replace={0}{}, % erase ’0’
        fixed zerofill,
        precision=2,
    },
    columns/3/.style={column name=,
        string replace={0}{}, % erase ’0’
        fixed zerofill,
        precision=2,
    },
    columns/4/.style={column name=,
        % string replace={0}{}, % erase ’0’
        fixed, fixed zerofill,
        precision=1,
        % postproc cell content/.style={@cell content/.add={}{\%}},
    },
    columns/5/.style={column name=,
        % string replace={0}{}, % erase ’0’
        fixed, fixed zerofill,
        precision=1,
        % postproc cell content/.style={@cell content/.add={}{\%}},
    },
    empty cells with={--}, % replace empty cells with ’--’
    %
    % For formatting individual cells:
    % Trained on same data:
    every row 1 column 0/.style={postproc cell content/.style={@cell content/.add={(}{)}}},
    every row 2 column 0/.style={postproc cell content/.style={@cell content/.add={(\boldmath}{)}}},
    every row 4 column 0/.style={postproc cell content/.style={@cell content/.add={(}{)}}},
    every row 11 column 0/.style={postproc cell content/.style={@cell content/.add={(}{)}}},
    every row 11 column 2/.style={postproc cell content/.style={@cell content/.add={(}{)}}},
    % Best values:
    every row 13 column 0/.style={postproc cell content/.style={@cell content/.add={\boldmath}{}}},
    every row 14 column 2/.style={postproc cell content/.style={@cell content/.add={\boldmath}{}}},
    every row 14 column 0/.style={postproc cell content/.style={@cell content/.add={\boldmath}{}}},
    every row 15 column 2/.style={postproc cell content/.style={@cell content/.add={\boldmath}{}}},
    every row 15 column 1/.style={postproc cell content/.style={@cell content/.add={\boldmath}{}}},
    every row 15 column 3/.style={postproc cell content/.style={@cell content/.add={\boldmath}{}}},
    every row 4 column 1/.style={postproc cell content/.style={@cell content/.add={\boldmath}{}}},
    every row 4 column 3/.style={postproc cell content/.style={@cell content/.add={\boldmath}{}}},
    % Percentages:
    every row 12 column 4/.style={postproc cell content/.style={@cell content/.add={}{\%}}},
    every row 13 column 4/.style={postproc cell content/.style={@cell content/.add={\boldmath}{\%}}},
    every row 14 column 4/.style={postproc cell content/.style={@cell content/.add={\boldmath}{\%}}},
    every row 15 column 4/.style={postproc cell content/.style={@cell content/.add={\boldmath}{\%}}},
    every row 12 column 5/.style={postproc cell content/.style={@cell content/.add={}{\%}}},
    every row 13 column 5/.style={postproc cell content/.style={@cell content/.add={}{\%}}},
    every row 14 column 5/.style={postproc cell content/.style={@cell content/.add={}{\%}}},
    every row 15 column 5/.style={postproc cell content/.style={@cell content/.add={\boldmath}{\%}}},
]{kitti_w_test.csv} % filename/path to file
\end{table*}

==> table_rgbdslam.tex <==
% http://pgfplots.sourceforge.net/pgfplotstable.pdf
\begin{table*}[!t]\centering
\caption{Performance comparison on the RGB-D SLAM dataset. We report the mean and median End Point Error (EPE) of the predicted optical flow,
the Percentage of Improved Instances (PoII) over the baseline model,
and the Mean Rotation Error (MRE) in degrees and Mean normalized Translation Error (MTE) of the estimated camera motion.
Results in parentheses indicate that the model was trained on that dataset.
%(without supervision).
PWC-Net is a supervised model pre-trained on the FlyingChairs and FlyingThings3D datasets.
EPIFlow-F* denotes the EPIFlow-F loss added to our baseline.
% Standard Deviation - move to suppl
% PWC-Net: 5.0336,7.8982
% EPIFlow: 5.791,9.6322
% Ours-Baseline: 5.083,9.1754
% Ours-ApproxGrad: 4.564,8.8579
% Ours-NoPrior: 4.565,8.9684
% Ours Train/Test: 4.481,8.9322
}
\label{tab:rgbdslam}
\newcolumntype{C}{>{\centering\arraybackslash}X}
% \renewcommand*{\arraystretch}{1.3} % Use/adjust if desired
\setlength{\tabcolsep}{0pt} % Use/adjust if desired
\begin{tabularx}{0.25\textwidth}{@{}l l}
    \toprule
    \\
    \addlinespace
    & Method\\
    \midrule
    \multirow{1}{10pt}{\rotatebox{90}{\small Su}}
    % &\small{Supervised}\\
    &PWC-Net \cite{sun2018pwc}\\
    \midrule
    \multirow{5}{10pt}{\rotatebox{90}{\small Unsupervised}}
    &EPIFlow-F* \cite{zhong2019unsupervised}\\
    % \cmidrule[\lightrulewidth](){2-2}
    \cmidrule[\lightrulewidth](r{-1.6em}){2-2}
    &Ours-Baseline\\
    &Ours-ApproxGrad\\
    &Ours-NoPrior\\
    &Ours\\
    \bottomrule
\end{tabularx}%
\pgfplotstabletypeset[
    column type=, % clear defaults
    trim cells=true,
    begin table={\begin{tabularx}{0.75\textwidth}{@{}C C C C C C C@{}}},
    % begin table={\begin{tabularx}{0.75\textwidth}{@{}C C C C C C C C C@{}}}, % With median
    end table={\end{tabularx}},
    col sep=comma,
    row sep=newline,
    header=false,
    every head row/.style={
        output empty row,
        before row={
            \toprule
            \multicolumn{2}{c}{EPE (mean) $\downarrow$} & \multicolumn{2}{c}{EPE (median) $\downarrow$} & PoII $\uparrow$ & MRE $\downarrow$ & MTE $\downarrow$\\
            % \multicolumn{2}{c}{EPE (mean)} & \multicolumn{2}{c}{EPE (median)} & PIF & MRE & MedRE & MTE & MedTE\\
            \cmidrule(lr){1-2}
            \cmidrule(lr){3-4}
            \cmidrule(lr){5-5}
            \cmidrule(lr){6-6}
            \cmidrule(lr){7-7}
            % \cmidrule(lr){8-8}
            % \cmidrule(lr){9-9}
            train & test & train & test & test & test & test\\
            % train & test & train & test & test & test & test & test & test\\
        },
        after row=\midrule,
    },
    every last row/.style={after row=\bottomrule},
    % every row no 0/.style={before row=\\},
    every row no 1/.style={before row=\midrule},
    every row no 2/.style={before row=\midrule},
    every row no 9/.style={before row=\midrule},
    %
    columns/0/.style={column name=,
        string replace={0}{}, % erase ’0’
        fixed, fixed zerofill,
        precision=2,
    },
    columns/1/.style={column name=,
        string replace={0}{}, % erase ’0’
        fixed, fixed zerofill,
        precision=2,
    },
    columns/2/.style={column name=,
        string replace={0}{}, % erase ’0’
        fixed, fixed zerofill,
        precision=2,
    },
    columns/3/.style={column name=,
        string replace={0}{}, % erase ’0’
        fixed, fixed zerofill,
        precision=2,
    },
    columns/4/.style={column name=,
        % string replace={0}{}, % erase ’0’
        fixed, fixed zerofill,
        precision=1,
        postproc cell content/.style={@cell content/.add={}{\%}},
    },
    columns/5/.style={column name=,
        string replace={0}{}, % erase ’0’
        fixed, fixed zerofill,
        precision=2,
    },
    columns/6/.style={column name=,
        string replace={0}{}, % erase ’0’
        fixed, fixed zerofill,
        precision=2,
    },
    columns/7/.style={column name=,
        string replace={0}{}, % erase ’0’
        fixed, fixed zerofill,
        precision=2,
    },
    columns/8/.style={column name=,
        string replace={0}{}, % erase ’0’
        fixed, fixed zerofill,
        precision=2,
    },
    % columns/9/.style={column name=,
    %     string replace={0}{}, % erase ’0’
    %     fixed, fixed zerofill,
    %     precision=2,
    % },
    empty cells with={--}, % replace empty cells with ’--’
    %
    % For formatting individual cells:
    % Trained on same data:
    every row 1 column 0/.style={postproc cell content/.style={@cell content/.add={(}{)}}},
    every row 2 column 0/.style={postproc cell content/.style={@cell content/.add={(}{)}}},
    every row 3 column 0/.style={postproc cell content/.style={@cell content/.add={(}{)}}},
    every row 4 column 0/.style={postproc cell content/.style={@cell content/.add={(}{)}}},
    every row 5 column 0/.style={postproc cell content/.style={@cell content/.add={(\boldmath}{)}}},
    every row 1 column 2/.style={postproc cell content/.style={@cell content/.add={(}{)}}},
    every row 2 column 2/.style={postproc cell content/.style={@cell content/.add={(}{)}}},
    every row 3 column 2/.style={postproc cell content/.style={@cell content/.add={(}{)}}},
    every row 4 column 2/.style={postproc cell content/.style={@cell content/.add={(}{)}}},
    every row 5 column 2/.style={postproc cell content/.style={@cell content/.add={(\boldmath}{)}}},
    % Best values:
    % every row 5 column 0/.style={postproc cell content/.append style={@cell content/.add={\boldmath}{}}},
    every row 5 column 1/.style={postproc cell content/.append style={@cell content/.add={\boldmath}{}}},
    % every row 5 column 2/.style={postproc cell content/.append style={@cell content/.add={\boldmath}{}}},
    every row 5 column 3/.style={postproc cell content/.append style={@cell content/.add={\boldmath}{}}},
    every row 5 column 4/.style={postproc cell content/.append style={@cell content/.add={\boldmath}{}}},
    every row 5 column 5/.style={postproc cell content/.append style={@cell content/.add={\boldmath}{}}},
    every row 5 column 6/.style={postproc cell content/.append style={@cell content/.add={\boldmath}{}}},
]{rgbdslam.csv} % filename/path to file
\end{table*}
